Decision-Making under Miscalibration

ML-based predictions are used to inform consequential decisions about individuals. How should we use predictions (e.g., risk of heart attack) to inform downstream binary classification decisions (e.g., undergoing a medical procedure)? When the risk estimates are perfectly calibrated, the answer is well understood: a classification problem's cost structure induces an optimal treatment threshold $j^{\star}$. In practice, however, some amount of miscalibration is unavoidable, raising a fundamental question: how should one use potentially miscalibrated predictions to inform binary decisions? We formalize a natural (distribution-free) solution concept: given anticipated miscalibration of $\alpha$, we propose using the threshold $j$ that minimizes the worst-case regret over all $\alpha$-miscalibrated predictors, where the regret is the difference in clinical utility between using the threshold in question and using the optimal threshold in hindsight. We provide closed form expressions for $j$ when miscalibration is measured using both expected and maximum calibration error, which reveal that it indeed differs from $j^{\star}$ (the optimal threshold under perfect calibration). We validate our theoretical findings on real data, demonstrating that there are natural cases in which making decisions using $j$ improves the clinical utility.

==> intro_draft.tex <==

\section{Introduction}

% things to include:
% - need to clarify the setup. e.g. once we have labeled data, can draw the Net Benefit and compare different models (based on j*, which is fixed). Emphasize that this is different from a usual setup for DS which is to choose the threhsold that optimizes the Net Benefit. can give the example of the task we worked with Clalit on, where the threshold is fixed at 7.5%. maybe look at that paper for a reference.
% - emphasize why it makes sense for our formulation to be this "worst-case"y. the issue is that we've exausted the development data (in terms of guaranteeing calibration), but still anticipate some miscalibration. the paper that proves the same result as us even goes further and recommends learning simple model to decrease the generalization error. 
% - future work: more complex calibration guarantees, and studying j_hat also as a function of p (assuming we have unlabeled data, so the mu's are fixed).

Powered by advances in machine learning, risk predictors are used to make and inform increasingly consequential decisions about individuals. A risk predictor maps an individual's features to an estimate of the probability that some event will occur, e.g. the individual will click on an ad, default on a loan, or experience a life-threatening cardiovascular event. These probabilities are then translated into binary decisions, or {\em classifications}: showing an ad, approving a loan, or perscribing a medical treatment. The costs of correct and incorrect classifications can vary wildly. For example, a false positive can be quite costly in the context of deciding on a medical treatment that has severe side effects. Indeed, a single risk predictor may be used for different decisions, e.g. deciding on different treatments, with varying costs (adverse side effects) and benefits (improved health outcomes). Given a problem's {\em cost structure}, consisting of numerical costs (or benefits) for true and false postive and negative classifications, we can quantify the {\em utility} (or the Net Benefit \cite{?}) of a classification model.  

If the predictions are calibrated, then, given the problem's cost structure, we can meaningfully translate the predictions into binary decisions. A (perfectly) calibrated predictor guarantees that, for each prediction ``category'' $v \in [0,1]$, of the individuals for whom the predicted risk was $v$, a $v$-fraction actually receive positive outcomes. Calibration is an important guarantee of meaninfulness for risk predictions \cite{David?}. Given calibrated predictions, we can treat individuals whose predicted risk exceeds the {\em therapeutic threshold} $\js$ \cite{?}: the smallest (true) risk level (true probability of a positive outcome) where treatment gives non-negative utility if the predictions are calibrated. \guy{refer to stronger guarantees (clinical harm)? Is there some prior formalization of why this is the optimal thing to do?}
On the other hand, if the predictor is mis-calibrated, then treating at the theraputic threshold can lead to (significant) negative utility. 

Thus, calibration is an important desideratum for risk models. In practice, however, \emph{some amount of miscalibration is unavoidable}, whether due to generalization errors or to distribution shifts. It is important to bound calibration errors, but they cannot be completely eliminated, and they can have a significant negative impact downstream, when the predictions are translated into decisions. The inevitability of calibration errors necessitates re-evaluating how risk predictions are translated into decisions. This is the starting point for our work.


\subsection{Our Contributions}
\label{sec:our-contributions}

We introduce and study a novel methodology for translating miscalibrated risk predictions into binary decisions. We study the following problem: given a risk predictor and a cost structure for the problem at hand, the goal is determining a risk threshold at which treatment should be applied. The true (target) distribution $D$ of individual-outcome pairs is unknown: all we know is a bound on the predictor's calibration error with respect to $D$. Using the therapeutic threshold may seem appealing, but as noted above, it can lead to negative utility. Indeed, depending on the direction of miscalibration errors, it might be better to treat at a higher or a lower risk threshold. 


For example, suppose that $\js=0.05$ is the theraputic threshold: individuals whose {\em true} risk (the probability of a positive outcome according to $D$) is 0.05 or higher will benefit from the treatment. This can happen if (and only if) the benefit from treating a true positive is 19 times larger than the harm from treating a true negative. With these costs in mind, should we treat individuals whose {\em predicted} risk is 0.04? If we were perfectly confident in our predictions, we wouldn't treat, but we anticipate some level of miscalibration. Importantly, the effects of calibration errors (overestimating or underestimating the risk) are not symmetrical. Suppose we don't these individuals, and later find out that their true risk was 0.14: we will have significant regret about our decision. On the other hand, if we treat them but later find out the true risk was 0, our regret will be much smaller. Given these complex considerations, what treatment threshold should we use?

\paragraph{Minimzing the worst-case regret.} We propose a new solution concept for deciding on the treatment threshold. Since the only thing we know about the target distribution is a bound on the miscalibration error, we propose that decisions should be made using the treatment threshold that minimizes the {\em worst-case regret} that might be incurred. For a threshold $j \in [0,1]$, given an alternative threshold $j' \in [0,1]$ and a distribution $D$ on individuals-outcome pairs, the regret for using $j$ rather than $j'$ is the difference between the utility obtained by threshold $j'$ and the utility obtained by $j$ (utility is measured over the distribution $D$). Let $\D_{\alpha}$ be the set of all distributions for which the predictor's miscalibration error (see below) is bounded by $\alpha$. The worst-case regret  for threshold $j \in [0,1]$ is the maximal regret that can be experienced, over all the possible alternative thresholds $j'$, and over all possible distributions $D' \in \D_{\alpha}$. See Definition \ref{?}.

%We elaborate on the latter point \guy{elaboration is unclear}: consider the individuals for whom the risk predictor predicted risk $v$.  Once $D'$ is fixed, it specifies the mass of this collection of individuals, as well as their true risk (the expected fraction of positive outcomes). If the true risk is not $v$, this contributes to the predictor's calibration error. Since we consider predictors whose calibration errors are bounded, we only enumerate over distributions whose errors are with that bound. \guy{perhaps say here that really what we care about in the distribution are the masses of each category and the calibration error.}

We emphasize two points: First, looking ahead, the theraputic threshold $\js$ does not always minimize the regret: it diverges from the regret-minimizing threshold when we anticipate errors ($\alpha > 0$), and the problem's cost structure is sufficiently asymetrical (see below). Second, our goal was deciding on a treatment threshold without knowing anything about the target distribution $D$, beyond the bound on the miscalibration error. The regret-minimizing threshold is thus, by design, a {\em distribution free} notion: it does not depend on the true distribution $D$. Rather, it is a function of the anticipated error rate $\alpha$ and of the cost structure (as manifested in the treatment threshold $\js$).

Regret is related to the notion of {\em Clinical Harm}: a performance measure from the decision-analytic literature \cite{?}. The clinical harm of a classification model is the difference between its utility and the utility of (the better of) two naive baselines: treating all individuals (treatment threshold 0) and treating none (threshold 1). We measure regret with respect to {\em all} possible alternative threshold (not just 0 and 1) and thus the regret for using a threshold is always at least as large as its clinical harm. Bounding the worst-case regret also implies bounds on the clinical harm. 

%\guy{Gal's text: Motivated by the above question, we generalize the notion of clinical harm to consider the regret against every fixed threshold (as opposed to just 0,1) and formalize a natural min-max objective: given $\alpha$ (anticipated miscalibration) and $\js$ (the therapeutic threshold, that implicitly captures the costs in question), choose the threshold $\hat{j}$ that minimzes the worst case regret (over all $\alpha$-miscalibrated predictors). }

\paragraph{Computing the regret-minimizing threshold.} We provide simple (and efficiently-computable) closed-form solutions for computing the regret-minimizing threshold, when the miscalibration is quantified using the standard measures of maximum and expected calibration errors (Definitions \ref{?} and \ref{?}). This is our main technical contribution. We note that the regret-minimizing threshold is the solution to a min-max problem over an exponential space of possibilities (in particular, the $\D_{\alpha}$ of all possible distributions that conform to the miscalibration bound), so it is infeasible to compute it by enumerating over all possibilities.

Our derivation highlights that the optimal threshold naturally follows a ``conservatism in the face of uncertainty'' approach. Recall the example above, where $\js=0.05$ and the predicted risk is 0.04: intuitively, it made sense to hedge our bets and treat these individuals, since the potential benfit if their risk was underestimated is much larger than the potential harm if the risk was over-estimated. The regret-minimizing threshold gives a rigorous explanation and formalization for this intuition.
\guy{do we want to call this the conservative therapeutic threshold?}

On a technical level, we obtain the closed-form expression in two steps. First, we show that the regret can always be maximized by a distribution that comes from a very restricted class, where all the individuals have one of (at most) two possible risk levels. We then derive a closed-form expression for computing a regret-minimizing threshold over this restricted class of distributions. See Section \ref{?} for further details.


% \paragraph{Implications for subgroup fairness.} Multicalibration (formally, a requirement that predictions be calibrated not only globally, but also simultaneously on a rich collection of protected demographic subgroups) is a popular notion of fairness in the algorithmic fairness community, starting with the work of \cite{hkrr}. Our work is motivated by and is closely related to these fairness concerns in two respects. First, the connection between calibration and decision-analytic notions such as Clinical Harm crystallize a specific subgroup harm that multi-calibrated predictions prevent: specifically, that there exists a protected groups for which using the predictor leads to utility that is worse than what was obtainable without the predictor. Second, our work provides a principled methodology for translating multi-calibrated predictions into decisions, minimizing the worst-case regret experienced by each of the subgroups.

\paragraph{Fairness and subgroup-utility.} 
As discussed above, calibration errors can lead to significant downstream harms. This raises a serious fairness concern: even if the predictions are globally calibrated, they can be significantly miscalibrated over protected demographic subgroups. Starting with \cite{?}, a series of recent works aim to obtain {\em multi-calibrated} risk predictors, whose calibration errors are bounded for rich collections of subgroups. Our work is motivated by these fairness concerns and these recent developments. We provide a principled methodology for translating multi-calibrated predictions into decisions, minimizing the worst-case regret experienced by each of the subgroups.



\paragraph{Conclusions and discussion.}
\guy{extensions: maybe we know *something* about the target distribution (e.g. unlabeled samples)}


==> shortened_abstract.tex <==

ML-based predictions are used to inform consequential decisions about individuals. How should we use predictions  (e.g., risk of heart attack) to inform downstream binary classification decisions (e.g., undergoing a medical procedure)? When the risk estimates are perfectly calibrated, the answer is well understood: a classification problem’s cost structure induces an optimal treatment threshold $\js$. %An individual should be treated if and only if their risk exceeds $\js$. 
In practice, however, some amount of miscalibration is unavoidable, raising a fundamental question: how should one use potentially miscalibrated predictions to inform binary decisions? 

We formalize a natural (distribution-free) solution concept: given anticipated miscalibration of $\alpha$, the optimal threshold $j$ is the one that minimizes the worst-case regret over all $\alpha$-miscalibrated predictors, where the regret is the difference in clinical utility between using the threshold in question and using the optimal threshold in hindsight. We provide closed form expressions for $j$ when miscalibration is measured using both expected and maximum calibration error, which reveal that it indeed differs from $\js$ (the optimal threshold under perfect calibration). We validate our theoretical findings on real data, demonstrating that there are natural cases in which making decisions using $j$ improves the clinical utility.
